Towards Battery-Free Wireless Sensing via Radio-Frequency Energy Harvesting

Diverse Wi-Fi-based wireless applications have been proposed, ranging from daily activity recognition to vital sign monitoring. Despite their remarkable sensing accuracy, the high energy consumption and the requirement for customized hardware modification hinder the wide deployment of the existing sensing solutions. In this paper, we propose REHSense, an energy-efficient wireless sensing solution based on Radio-Frequency (RF) energy harvesting. Instead of relying on a power-hungry Wi-Fi receiver, REHSense leverages an RF energy harvester as the sensor and utilizes the voltage signals harvested from the ambient Wi-Fi signals to enable simultaneous context sensing and energy harvesting. We design and implement REHSense using a commercial-off-the-shelf (COTS) RF energy harvester. Extensive evaluation of three fine-grained wireless sensing tasks (i.e., respiration monitoring, human activity, and hand gesture recognition) shows that REHSense can achieve comparable sensing accuracy with conventional Wi-Fi-based solutions while adapting to different sensing environments, reducing the power consumption by 98.7% and harvesting up to 4.5mW of power from RF energy.

==> algorithms/meta-training-alg.tex <==
\begin{algorithm}[t]
\caption{Meta-training for adapting HAR/HGR classifiers to other conditions}
\label{alg:meta-training}
\small
\DontPrintSemicolon

\KwIn{$\mathcal{D}_{S_{a}}$, $\mathcal{D}_{S_{g}}$: source datasets of HAR and HGR. $f_{a}$, $f_{g}$: classifiers of HAR and HGR. $\alpha_{a}$, $\alpha_{g}$ and $\beta_{a}$, $\beta_{g}$: training hyperparameters of HAR and HGR.}

\KwOut{$f_{\theta^{*}_{a}}$, $f_{\theta^{*}_{g}}$: trained HAR classifier and HGR classifier with optimized parameters $\theta^{*}_{a}$ and $\theta^{*}_{g}$.}

$\theta_{a}\leftarrow \theta_{a_{0}}$, $f_{\theta_{a}}\leftarrow f_{\theta_{a_{0}}}$ \algorithmiccomment{random initialize HAR classifier $f_{\theta_{a}}$ with parameters $\theta_{a_{0}}$}.

$\theta_{g}\leftarrow \theta_{g_{0}}$, $f_{\theta_{g}}\leftarrow f_{\theta_{g_{0}}}$ \algorithmiccomment{random initialize HGR classifier $f_{\theta_{g}}$ with parameters $\theta_{g_{0}}$}.

\While{not finished} {

$\mathcal{T}_{a}, \mathcal{T}_{g}\leftarrow$ generate a batch of HAR and HGR tasks from $\mathcal{D}_{S_{a}}$ and $\mathcal{D}_{S_{g}}$.

\For{each task $\mathcal{T}_{a_{i}}\in\mathcal{T}_{a}$, $\mathcal{T}_{g_{i}}\in\mathcal{T}_{g}$}{

$\mathcal{S}_{\mathcal{T}_{a_{i}}}\leftarrow K_{a}\times N_{a}$ support samples from $\mathcal{T}_{a_{i}}$.

$\mathcal{S}_{\mathcal{T}_{g_{i}}}\leftarrow K_{g}\times N_{g}$ support samples from $\mathcal{T}_{g_{i}}$.

$\mathcal{Q}_{a_{i}}\leftarrow K_{a}\times N_{a}$ query samples from $\mathcal{T}_{a_{i}}$ ($\mathcal{S}_{\mathcal{T}_{a_{i}}}\cap \mathcal{Q}_{a_{i}}=\phi$)

$\mathcal{Q}_{g_{i}}\leftarrow K_{g}\times N_{g}$ query samples from $\mathcal{T}_{g_{i}}$ ($\mathcal{S}_{\mathcal{T}_{g_{i}}}\cap \mathcal{Q}_{g_{i}}=\phi$)

Evaluate $\nabla_{\theta_{a}}\mathcal{L}_{\mathcal{T}_{a_{i}}}(f_{\theta_{a}})$, $\nabla_{\theta_{g}}\mathcal{L}_{\mathcal{T}_{g_{i}}}(f_{\theta_{g}})$ with $\mathcal{S}_{\mathcal{T}_{a_{i}}}$, $\mathcal{S}_{\mathcal{T}_{g_{i}}}$ and loss $\mathcal{L}_{\mathcal{T}_{a_{i}}}(f_{\theta_{a}}, \mathcal{S}_{\mathcal{T}_{a_{i}}})$, $\mathcal{L}_{\mathcal{T}_{g_{i}}}(f_{\theta_{g}}, \mathcal{S}_{\mathcal{T}_{g_{i}}})$

$\tilde{\theta}_{\mathcal{T}_{a_{i}}}\leftarrow\theta_{a_{0}}-\alpha_{a}\nabla_{\theta_{a}}\mathcal{L}_{\mathcal{T}_{a_{i}}}(f_{\theta_{a_{0}}}, \mathcal{S}_{\mathcal{T}_{a_{i}}})$, $\tilde{\theta}_{\mathcal{T}_{g_{i}}}\leftarrow\theta_{g_{0}}-\alpha_{g}\nabla_{\theta_{g}}\mathcal{L}_{\mathcal{T}_{g_{i}}}(f_{\theta_{g_{0}}}, \mathcal{S}_{\mathcal{T}_{g_{i}}})$ \algorithmiccomment{obtain task-specific parameters $\tilde{\theta}_{\mathcal{T}_{a_{i}}}$, $\tilde{\theta}_{\mathcal{T}_{g_{i}}}$ of $\mathcal{T}_{a_{i}}$, $\mathcal{T}_{g_{i}}$ using gradient descent.}

Evaluate $\mathcal{L}_{\mathcal{T}_{a_{i}}}(f_{\tilde{\theta}_{\mathcal{T}_{a_{i}}}})$, $\mathcal{L}_{\mathcal{T}_{g_{i}}}(f_{\tilde{\theta}_{\mathcal{T}_{g_{i}}}})$ with query set $\mathcal{Q}_{a_{i}}$, $\mathcal{Q}_{g_{i}}$.
}
$\theta^{*}_{a}\leftarrow \theta_{a_{0}}-\beta_{a}\nabla_{\theta_{a}}\sum_{\mathcal{T}_{a_{i}}\in\mathcal{T}_{a}}\mathcal{L}_{\mathcal{T}_{a_{i}}}(f_{\tilde{\theta}_{\mathcal{T}_{a_{i}}}}, \mathcal{Q}_{a_{i}})$, $\theta^{*}_{g}\leftarrow \theta_{g_{0}}-\beta_{g}\nabla_{\theta_{g}}\sum_{\mathcal{T}_{g_{i}}\in\mathcal{T}_{g}}\mathcal{L}_{\mathcal{T}_{g_{i}}}(f_{\tilde{\theta}_{\mathcal{T}_{g_{i}}}}, \mathcal{Q}_{g_{i}})$. \algorithmiccomment{obtain the optimized parameters $\theta^{*}_{a}$, $\theta^{*}_{g}$ that minimizes all task losses.}
}

Output HAR and HGR classifiers $f_{\theta^{*}_{a}}$, $f_{\theta^{*}_{g}}$ with optimized parameters $\theta^{*}_{a}$, $\theta^{*}_{g}$.
\end{algorithm}

==> tables/comparison-energy-consumption.tex <==
\begin{table}[t]
\centering
\caption{Energy consumption.}
\label{tab:comparison-energy-consumption}
\scriptsize
\setlength{\tabcolsep}{4pt}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{ccc}
\toprule
\textbf{System} & \textbf{Component} & \textbf{Power Consumption} \\ \midrule
\multirow{2}{*}{REHSense} & P21XXCSR-EVB board & \SI{0}{\milli\watt} (Passive) \\ \cmidrule{2-3} 
 & Arduino Nano and MicroSD card & $11.3-$\SI{12.6}{\milli\watt} \\ \midrule
\multirow{2}{*}{CSI-based} & Intel 5300 NIC card & $820-$\SI{940}{\milli\watt}~\cite{halperin2010demystifying}~\cite{jang2011snooze}\\ \cmidrule{2-3} 
 & Lenovo T400 laptop & $16.3\times 10^{3}-38.8\times 10^{3}$\SI{}{\milli\watt} \\ \bottomrule
\end{tabular}%
%}
\end{table}
